Leveraging translations for speech transcription in low-resource settings

Recently proposed data collection frameworks for endangered language documentation aim not only to collect speech in the language of interest, but also to collect translations into a high-resource language that will render the collected resource interpretable. We focus on this scenario and explore whether we can improve transcription quality under these extremely low-resource settings with the assistance of text translations. We present a neural multi-source model and evaluate several variations of it on three low-resource datasets. We find that our multi-source model with shared attention outperforms the baselines, reducing transcription character error rate by up to 12.3%.

==> mboshi.tex <==
\begin{table}[th]
    \centering
    \begin{tabular}{c|c|ccc|cc}
    \toprule
        \multirow{3}{*}{} & \multicolumn{5}{c}{Mboshi} \\
         & char & \multicolumn{3}{c}{char+seg} & \multicolumn{2}{|c}{word} \\
         & CER & CER & WER & BLEU & WER & BLEU \\
    \midrule
        speech & 42.1 & 50.1 & 63.4 & 20.1 & 100 & 3.0\\
        translation (c) & 73.3 & 87.9 & 91.7 & 6.7 & 99.5 & 5.3\\
        translation (w) & 69.3 & 87.1 & 89.7 & 8.0 & 93.6 & 6.4\\
    \midrule
        speech+translation(c) & 71.6 & 83.5 & 88.2 & 7.8 & 96.05 & 4.2\\
        speech+translation(w) & 68.9 & 60.5 & 73.1 & 14.1 & 93.6 & 6.7\\
    \bottomrule     
    \end{tabular}
    \caption{Error Rates on Mboshi when decoding at the character level, character level with word segmentation information, and at the word level.}
    \label{tab:mb_cer_results}
\end{table}
